MCiteBench: A Multimodal Benchmark for Generating Text with Citations

Multimodal Large Language Models (MLLMs) have advanced in integrating diverse modalities but frequently suffer from hallucination. A promising solution to mitigate this issue is to generate text with citations, providing a transparent chain for verification. However, existing work primarily focuses on generating citations for text-only content, leaving the challenges of multimodal scenarios largely unexplored. In this paper, we introduce MCiteBench, the first benchmark designed to assess the ability of MLLMs to generate text with citations in multimodal contexts. Our benchmark comprises data derived from academic papers and review-rebuttal interactions, featuring diverse information sources and multimodal content. Experimental results reveal that MLLMs struggle to ground their outputs reliably when handling multimodal input. Further analysis uncovers a systematic modality bias and reveals how models internally rely on different sources when generating citations, offering insights into model behavior and guiding future directions for multimodal citation tasks.

==> 080ethics.tex <==
We hereby acknowledge that all authors of this work are aware of the provided ACL Code of Ethics and honor the code of conduct.

\paragraph{Use of Human Annotations}
Our institution recruited three annotators to perform the evidence linking, data filtering, and robustness evaluation tasks for \method. We ensure that the privacy rights of the annotators are respected throughout the process. The annotators receive compensation exceeding the local minimum wage and have consented to participate in the tasks for research purposes.


\paragraph{Risks}
The tasks in \method used in our experiment are created by human annotators, and we conduct additional checks to ensure that the content is free from socially harmful or toxic language. However, the evaluation of data quality relies on common sense, which may differ across individuals with diverse backgrounds.

==> list/quality_protocol_explanation.tex <==
\begin{table*}[!htbp]
\begin{tcolorbox}
I. Question Quality

A. Relevance and Intent

Positive Rules:

Questions should be directly related to the content of the paper, specifically pointing to a particular section, method, result, or statement in the paper, seeking clarification, detailed information, or a deeper understanding of specific content.

Example: "In Section 3.1, why did you choose to use KL divergence to analyze model performance?"

Negative Rules:

Avoid questions that include suggestions, opinions, or feedback, such as proposing improvements to experiments, methods, or suggesting new ideas.

Example: "Have you considered adding more datasets in future work?"

Avoid asking authors to make subjective speculations or explanations beyond the scope of the paper, such as inquiring about content not discussed in the paper, future possibilities, or the authors' personal viewpoints.

Example: "Do you think your method is applicable in other fields?"
Avoid overly broad or general questions that cannot find a clear answer in the paper.

Example: "What are the contributions of your method?"

Avoid asking about issues not explicitly explained or analyzed in the paper, especially when the answer would require authors to make additional conjectures.

Example: "Why does your adaptive constraint improve performance?"

B. Clarity and Specificity

Positive Rules:

Questions should be clear and specific, pointing precisely to a detail in the paper, enabling readers to accurately understand the content the question targets.

Example: "In Figure 5, what factors contributed to the performance drop of Model A?"

Negative Rules:

Avoid ambiguous or unclear questions that make it impossible to determine the specific content being asked.

Example: "Can you explain in detail?"

Avoid overly broad questions that lack specific details and cannot find a clear answer in the paper.

Example: "Can you talk about your findings?"
C. Answerability

Positive Rules:

Questions should be answerable, with answers that can be directly found in the paper or clearly explained by the authors.

Example: "In your experiments, did you compare the performance of Method X and Method Y? What were the results?"

Negative Rules:

Avoid asking questions for which answers cannot be found in the paper, such as inquiring about unreported experiments, data, or viewpoints not discussed by the authors.

Example: "Did you test your model with different parameter settings?"
II. Overall Applicability of the QA Pair
A. Contribution to Evaluation

Positive Rules:
The QA pair should help assess the model's ability to understand and reason about the content of the paper, involving specific, verifiable knowledge points and testing the model's reading comprehension and information retrieval capabilities.

Negative Rules:
Avoid QA pairs that cannot be used to evaluate the model's understanding ability, such as questions that are too simple, overly broad, or involve content beyond the scope of the paper.

Avoid open-ended questions or those that require subjective speculation, as they are difficult to effectively reflect in model evaluation.

B. Exclusion Criteria
Suggestive Questions
Exclude questions that include suggestions, opinions, or feedback, as they do not test the model's understanding and reasoning abilities.

Example: "I suggest adding more datasets to your experiments."

Subjective Speculative Questions

Exclude questions that require authors to make subjective speculations or discuss content not covered in the paper.

Example: "Do you think this method will be applied in other fields in the future?"
Overly Broad or Ambiguous Questions

Exclude questions for which a clear answer cannot be found in the paper.

Example: "Can you explain in detail?"

Questions Beyond the Paper's Content

Avoid asking about issues not explicitly explained or analyzed in the paper; if the answer requires authors to make additional conjectures or explanations, it should be considered low quality.

Example: "Why does your proposed method improve performance while others do not?"

Inquiries About Unreported Experiments or Results

Avoid asking about experiments, data, or results not reported in the paper.

Example: "Did you test the performance of your model on large datasets?"

III. Final Summary

By integrating and refining the above rules, we aim to ensure that the QA pairs included in the benchmark possess the following characteristics:

Questions:

Clear and specific, directly related to the content of the paper.
Answers can be found explicitly in the paper, without requiring authors to make additional conjectures or subjective explanations.

Overall Applicability:

Helps evaluate the model's ability to understand and reason about the content of the paper, involving specific knowledge points and information retrieval.

QA pairs to be avoided include:

Questions that include suggestions, opinions, or feedback.

Questions that require authors to make subjective speculations or discuss content not covered in the paper.

Overly broad, ambiguous, or questions for which answers cannot be found in the paper.

Questions that require authors to make additional conjectures or explanations not explicitly provided in the paper.

\caption{Quality protocol for model-filtered and human-verified data.}
\label{prompt:quality_protocol_explanation}
\end{tcolorbox}
\end{table*}

==> table/attribution_vs_understanding.tex <==
\begin{table}[t]
  \centering
  \small
  \begin{tabular}{lcc}
    \toprule
    \textbf{Model}
    & \textbf{Understanding}
    & \textbf{Attribution} \\
    \midrule
    \textcolor{gray!50}{\textbf{Open-Source(7-14B)}} \\
    Qwen2-VL-7B       & 0.94 & 0.59   \\
    InternVL2\_5-8B       & 0.91 & 0.56   \\
    \textcolor{gray!50}{\textbf{Open-Source(>70B)}} \\
    Qwen2-VL-72B      & 0.95 & 0.62   \\
    InternVL2\_5-78B     & 0.93 & 0.62   \\
    \textcolor{gray!50}{\textbf{Proprietary}} \\
    GPT-4o-mini       & 0.93 & 0.61   \\
    GPT-4o       & 0.94 & 0.63   \\
    \bottomrule
  \end{tabular}
  \caption{Comparison of model performance on Understanding and Attribution tasks.}
  \label{tab:Attribution_or_Understanding}
\end{table}

==> table/exp_1.tex <==
\begin{table*}[t]
  \centering
  \small
  \begin{tabular}{lBBddqqBBddqq}
    \toprule
    \multirow{3}{*}{\textbf{Model}}
    & \multicolumn{6}{c}{\textbf{Subjective}}
    & \multicolumn{6}{c}{\textbf{Objective}} \\
    \cmidrule(lr){2-7} \cmidrule(lr){8-13}
    & \multicolumn{2}{c}{\textbf{5 Sample}}
    & \multicolumn{2}{c}{\textbf{10 Sample}}
    & \multicolumn{2}{c}{\textbf{15 Sample}}
    & \multicolumn{2}{c}{\textbf{5 Sample}}
    & \multicolumn{2}{c}{\textbf{10 Sample}}
    & \multicolumn{2}{c}{\textbf{15 Sample}} \\
    \cmidrule(lr){2-3} \cmidrule(lr){4-5} \cmidrule(lr){6-7} \cmidrule(lr){8-9} \cmidrule(lr){10-11} \cmidrule(lr){12-13}
    & \multicolumn{1}{c}{\textbf{F1}}
    & \multicolumn{1}{c}{\textbf{Acc.}}
    & \multicolumn{1}{c}{\textbf{F1}}
    & \multicolumn{1}{c}{\textbf{Acc.}}
    & \multicolumn{1}{c}{\textbf{F1}}
    & \multicolumn{1}{c}{\textbf{Acc.}}
    & \multicolumn{1}{c}{\textbf{F1}}
    & \multicolumn{1}{c}{\textbf{Acc.}}
    & \multicolumn{1}{c}{\textbf{F1}}
    & \multicolumn{1}{c}{\textbf{Acc.}}
    & \multicolumn{1}{c}{\textbf{F1}}
    & \multicolumn{1}{c}{\textbf{Acc.}} \\
    \midrule
    \textcolor{gray!50}{\textbf{Open-Source(7-14B)}} \\
    Qwen2-VL-7B       & 67.28 & 55.5  & 58.05 & 55.33 & 56.81 & 54.5  & 55.09 & 89.33 & 44.34 & 89.33 & 41.18 & 88.17 \\
    InternVL2\_5-8B   & 69.45 & 58.67 & 69.18 & 58.5  & 64.45 & 58.67 & 66.11 & 89    & 64.37 & 88.83 & 61.59 & 87.25 \\
    \textcolor{gray!50}{\textbf{Open-Source(>70B)}} \\
    Qwen2-VL-72B      & 66.58 & 56.83 & 62.22 & 54.67 & 63.95 & 56    & 70.12 & 92.83 & 64.66 & 91.33 & 56.42 & 90.67 \\
    InternVL2\_5-78B  & 70.92 & 60    & 79.89 & 60.83 & 82.23 & 60.33 & 60.95 & 93    & 58.64 & 92    & 63.21 & 92.5  \\
    \textcolor{gray!50}{\textbf{Proprietary}} \\
    GPT-4o-mini       & 64.29 & 62.17 & 71.7  & 60    & 71.87 & 62.17 & 69.84 & 92.42 & 63    & 91.67 & 66.76 & 91    \\
    GPT-4o-2024-11-20 & 83.87 & 69.33 & 83.41 & 68.33 & 84.39 & 70.17 & 89.43 & 93.67 & 88.39 & 92.08 & 87.74 & 92.42 \\
    \bottomrule
  \end{tabular}
  \caption{Comparison of different models on subjective and objective tasks.}
  \label{tab:exp_1}
\end{table*}

==> table/exp_2.tex <==
% \newcolumntype{g}{>{\columncolor{green!4}}c}
% \newcolumntype{r}{>{\columncolor{red!4}}c}
% \cellcolor{red!4}
% \cellcolor{green!4}
\begin{table*}[t]
  \centering
  \small
  \begin{tabular}{lcccccc}
    \toprule
    \multirow{2}{*}{\textbf{Model}}
    & \multicolumn{3}{c}{\textbf{Subjective}}
    & \multicolumn{3}{c}{\textbf{Objective}} \\
    \cmidrule(lr){2-4} \cmidrule(lr){5-7}
    & \multicolumn{1}{c}{\textbf{w/o citation}}
    & \multicolumn{1}{c}{\textbf{w/ citation}}
    & \multicolumn{1}{c}{\textbf{percentage}}
    & \multicolumn{1}{c}{\textbf{w/o citation}}
    & \multicolumn{1}{c}{\textbf{w/ citation}}
    & \multicolumn{1}{c}{\textbf{percentage}} \\
    \midrule
    \textcolor{gray!50}{\textbf{Open-Source(7-14B)}} \\
    Qwen2-VL-7B       & 51.33&51.5&\cellcolor{green!4}0.33&85.33&87.5&\cellcolor{green!4}2.54 \\
    InternVL2\_5-8B   & 51.58&51.83&\cellcolor{green!4}0.48&83.67&84.5&\cellcolor{green!4}0.99 \\
    \textcolor{gray!50}{\textbf{Open-Source(>70B)}} \\
    Qwen2-VL-72B      & 51.08&52.33&\cellcolor{green!4}2.45&87.0&89.67&\cellcolor{green!4}3.07 \\
    InternVL2\_5-78B  & 53.75&53.0&\cellcolor{red!4}-1.4&88.33&89.17&\cellcolor{green!4}0.95 \\
    \textcolor{gray!50}{\textbf{Proprietary}} \\
    GPT-4o-mini       & 53.25&53.0&\cellcolor{red!4}-0.47&86.5&87.0&\cellcolor{green!4}0.58 \\
    GPT-4o-2024-11-20 & 55.92&54.0&\cellcolor{red!4}-3.43&89.5&89.67&\cellcolor{green!4}0.19  \\
    \bottomrule
  \end{tabular}
  \caption{Evaluating the impact of explicit citation usage on answer accuracy across three experimental settings: answers without citation, answers with citation. The comparison examines whether citations enhance response accuracy or influence model performance consistency. }
  \label{tab:exp_2}
\end{table*}
